Bridging the Gap between Expert and Language Models: Concept-guided Chess Commentary Generation and Evaluation

Deep learning-based expert models have reached superhuman performance in decision-making domains such as chess and Go. However, it is under-explored to explain or comment on given decisions although it is important for model explainability and human education. The outputs of expert models are accurate, but yet difficult to interpret for humans. On the other hand, large language models (LLMs) can produce fluent commentary but are prone to hallucinations due to their limited decision-making capabilities. To bridge this gap between expert models and LLMs, we focus on chess commentary as a representative task of explaining complex decision-making processes through language and address both the generation and evaluation of commentary. We introduce Concept-guided Chess Commentary generation (CCC) for producing commentary and GPT-based Chess Commentary Evaluation (GCC-Eval) for assessing it. CCC integrates the decision-making strengths of expert models with the linguistic fluency of LLMs through prioritized, concept-based explanations. GCC-Eval leverages expert knowledge to evaluate chess commentary based on informativeness and linguistic quality. Experimental results, validated by both human judges and GCC-Eval, demonstrate that CCC generates commentary which is accurate, informative, and fluent.

==> arxiv/03method.tex <==

% \section{Chess Commentary Generation with Concept-based Explanation}
\section{Concpet-guided Chess Commentary Generation via LLM and Expert Model}

We propose Concept-guided Chess Commentary generation (\texttt{CCC}), which is a method for generating chess commentary by leveraging a chess expert model and its concept-based explanations. Figure~\ref{fig:method_overview} illustrates \texttt{CCC}.
This section consists of the definition of concepts (Section~\ref{subsec:concept}), the generation of concept-based explanation (Section~\ref{subsec:concept_explanation}), the prioritization of concepts (Section~\ref{subsec:prioritization}), and LLM-based generation using the expert model (Section~\ref{subsec:prompt_engineering}).

\subsection{Concept}
\label{subsec:concept}

Concepts are high-level abstractions of knowledge commonly shared within a community.
We highlight two key properties of concepts:
i) Concepts enable efficient communication by allowing the omission of verbose explanations. 
For instance, if someone want to explain an attack plan without the concept of "king safety", one should explain all potential threats against the king, threats to nearby squares and corresponding defense plans. 
Communication becomes more efficient and concise with concepts.
ii) Concepts are understandable to both humans and language models. 
Language models are trained in human text and share an understanding of concepts. 
The idea of concept-based explanation is to make a neural network interpretable by aligning it with a shared understanding of concepts.


\subsection{Learning Concepts-based Explanation}
\label{subsec:concept_explanation}

Concept-based explanation is finding a concept vector in the representation space of a model, and revealing the internal decision-making process of the model.
This approach relies on an assumption that concepts are embedded in the representation space~\cite{TCAV, mcgrath2022acquisition, gurnee2023finding, nanda_othello_2023}.
We further assume that the concept vector is linear, which is empirically supported by \citet{TCAV, mcgrath2022acquisition, gurnee2023finding, tenney2019bert, nanda_othello_2023}.
The assumption is validated for chess expert models, specifically, \texttt{Stockfish 14}~\cite{stockfish} and \texttt{AlphaZero}~\cite{alphazero} by \citet{ijcai2023stockfish} and \citet{mcgrath2022acquisition}, respectively.
We use \texttt{LeelaChessZero T78}~\cite{lc0}, which is an open-source version that shares the key structure of \texttt{AlphaZero}.

A common approach~\cite{TCAV, yuksekgonul23posthoc} to learn concept vectors consists of two steps: preparing concept labels or datasets, and finding a concept vector via optimization or training a classification model.
The list of concepts, in Table~\ref{tab:concept_result}, is adopted from \texttt{Stockfish 8}, which is a classical chess engine. 
For the concept learning dataset, we collected 200,000 chess positions from Lichess open database~\footnote{\url{https://database.lichess.org/\#evals}}, and for each concept, gather the top-$5\%$ of the data as positive samples and bottom-$5\%$ of the data as negative samples based on \texttt{Stockfish 8} evaluations.
For the representation space of \texttt{LeelaChessZero T78}, we use layer 40, which is the last layer of the residual blocks, just before separated into policy head and value head.
To extract concept vectors, we train a linear Support Vector Machine (SVM)~\citep{svm}, classifying the positive and negative samples in representation space.
We use the normal vector of the linear classification boundary as a concept vector, and the distance from the classification boundary plane of an input to be a concept score for the input.



\subsection{Prioritization of Concepts}
\label{subsec:prioritization}

While we can extract concept scores for every concept, concept scores do not directly indicate the importance of a concept in explaining a specific move.
For example, if a player has a well-positioned, powerful bishop, the bishop might be considered valuable and highlighted, even if the player does not move the bishop for several moves.
We define the priority of concept using improvement of concept score after a move and its response.
Since chess is a turn-based game, the position after a move becomes the turn of the opponent.
The concept score from the opponent's turn is different because an advantage of white is a disadvantage of black.
Thus, we compare the concept score after opponent's move, with the assumption that the opponent always plays optimal move.
By comparing the post-move and pre-move positions, we determine the influence of the move on each concept, thereby assigning priority to the most significantly affected concepts for the move.


\subsection{LLM-based Commentary Generation}
\label{subsec:prompt_engineering}

We generate chess commentary using an LLM and a chess expert model.
Although a language model understands chess specific notations and terms, it lacks the ability to perform chess-specific reasoning and complex analysis, which leads to hallucination.
By integrating chess expert model output, the LLM decides whether to focus on advantageous aspects or disadvantageous aspects.
However, since the chess expert model output is based on scalar values, it still generates incorrect comments.
Concept-based explanation guides the LLM to focus on critical aspects.
Figure~\ref{fig:comment_examples} shows a typical example of a concept-guided comments.

To enhance the reasoning ability of LLM, we employed few-shot prompting, Chain-of-Thought (CoT) prompting~\cite{wei2022chain}, and chess-specific information.
This approach provides the LLM with a deeper understanding of chess positions, and prevents potential use of wrongly prioritized concepts.
Additionally, we enumerate all existing attacks towards opponent pieces to prevent mentioning of non-existing pieces or illegal moves.



\section{Automatic Evaluation of Chess Commentary}
\label{sec:auto_eval_chess_comment}

Evaluating a chess commentary is a complex task.
Commentaries for the same position can be diverse, and may focus on different aspects such as an advantage on the kingside, an opponent's weakness, defensive plans, or the reasoning behind not selecting a different move.
Evaluating commentary also requires chess knowledge, because without it, judging the correctness or relevance of a sentence to the given move is impossible.

\citet{jhamtani18gac, zang19scc, lee2022meta} use classical metrics such as BLEU, ROUGE, and METEOR, which are based on language similarity to reference, or perplexity, which is a confidence of language model. 
However, these metrics are insufficient for judging chess commentaries.
While the ideal evaluation is the manual evaluation by a human expert, 
we propose an automatic evaluation metric using an LLM.

We build upon recent advancements in LLM-based natural language generation evaluation methodologies~\cite{bertscore, unieval, geval} that have been successfully employed in summarization and translation, which face similar challenges. 
Specifically, we adopt and extend the \texttt{G-Eval}~\cite{geval}, an LLM-based evaluation model that generates integer scores and addresses the challenge of producing non-integer values by computing a weighted sum of score tokens based on their probabilities:

\begin{align}
\mathrm{score}(x) = \sum_{s \in \{1,2,3,4,5\}}{s \times p(s | x)}   .  
\end{align}

While \texttt{G-Eval} provides a solid foundation, it still lacks the domain-specific knowledge required for evaluating chess commentary. 
To address this, we propose \texttt{G-Eval-CC} (\texttt{G-Eval} for chess commentary), which integrates essential chess knowledge as additional input to the model. 
This includes incorporating attack patterns and expert model evaluations to inform the chess-specific knowledge. 
This additional information enable the model to better align its scoring with expert-level chess understanding.
We describe the prompts in Appendix~\ref{sec:appendix_G_eval_cc}.

We focus on two key aspects of commentary evaluation: relevance and completeness, as correctness is inadequate for evaluation by an LLM, and linguistic evaluations, such as clarity and fluency are relatively trivial. 
For these metrics, expert model evaluations, alongside reference comments, are provided to guide the LLM. 
This enables the model to assess whether the commentary adequately addresses the important aspects of the position or move. 
The effectiveness of our approach for relevance, completeness, clarity, and fluency is verified in Section~\ref{subsec:exp_auto_eval}.
For correctness, where the accuracy of individual statements is paramount, we do not rely on LLM-based evaluation. 
We find that LLMs do not possess the required depth of chess knowledge, even when provided with additional expert model evaluation, to accurately evaluate correctness without significant human guidance. 


==> fig-tab/fig_concept_generation_prompt.tex <==

\begin{figure*}[t]
    \centering
    
    \begin{tcolorbox}[colback=mybrown!5!white,colframe=mybrown!75!black]
    \begin{small}
    \textbf{[System]}\\
    This is a chess commentary assistant consists of board, move, evaluation by stockfish, important concept candidates, concept evaluation and comment. \\
    {\color{blue}
    \textbf{[User]}\\
    board: 2rqrbk1/pp3ppp/8/3p1N2/3NnnQ1/2P4P/PP3PP1/R4RK1 w - - 0 23 \\
    actual move: 23. Nh6+ \\
    evaluation: actual move - Nh6+ 468cp, best move - Nh6+ 511cp, second best move - Qxf4 -25cp \\
    \underline{concept candidates}: pin, Black queen, White rook \\
    \textbf{[Assistant]}\\
    \underline{concept evaluation}: pin - g7 pawn is pinned and cannot capture the knight. \emph{...(omitted)...} \\
    comment: nice move, plan to fork king and queen Nh6+ and Nf7+, and black cannot capture knight because of pin . \\
    }
    \emph{...(omitted)...} \\
    \textbf{[User]}\\
    board: 8/1bp4p/p3P1p1/3n4/3kN1P1/5P1P/P1P2K2/8 b - - 0 0 \\
    actual move: 27... Ne7 \\
    evaluation: actual move - Ne7 301cp, expected reply - e4f6, best move - Bc8 358cp, second best move - h6 285cp \\
    concept candidates: Black Knights, White Passedpawns, Black Kingsafety \\
    \end{small}
    \end{tcolorbox}
    \caption{Prompt for generation using concepts. 
    The blue colored texts are few-shot prompting. In the real prompt, the other examples are omitted because of the length
    The underlined text are self-reasoning of the language model.
    }
\end{figure*}

